DeepStability: A Study of Unstable Numerical Methods and Their Solutions in Deep Learning

Deep learning (DL) has become an integral part of solutions to various important problems, which is why ensuring the quality of DL systems is essential. One of the challenges of achieving reliability and robustness of DL software is to ensure that algorithm implementations are numerically stable. DL algorithms require a large amount and a wide variety of numerical computations. A naive implementation of numerical computation can lead to errors that may result in incorrect or inaccurate learning and results. A numerical algorithm or a mathematical formula can have several implementations that are mathematically equivalent, but have different numerical stability properties. Designing numerically stable algorithm implementations is challenging, because it requires an interdisciplinary knowledge of software engineering, DL, and numerical analysis. In this paper, we study two mature DL libraries PyTorch and Tensorflow with the goal of identifying unstable numerical methods and their solutions. Specifically, we investigate which DL algorithms are numerically unstable and conduct an in-depth analysis of the root cause, manifestation, and patches to numerical instabilities. Based on these findings, we launch, the first database of numerical stability issues and solutions in DL. Our findings and provide future references to developers and tool builders to prevent, detect, localize and fix numerically unstable algorithm implementations. To demonstrate that, using {\it DeepStability} we have located numerical stability issues in Tensorflow, and submitted a fix which has been accepted and merged in.

==> background.tex <==
\section{Background}
\subsection{Numerical Stability}
% Numerical stability concerns how errors introduced during the execution of an algorithm affect the result. It is a property of an algorithm rather than the problem being solved \cite{Higham2002AccuracyAS}. It represents the sensitivity and robustness of the algorithm to errors introduced in inputs or intermediate results. A numerically stable algorithm does not amplify errors and therefore; errors do not have a significant impact on the final result.
% Numerical stability research papers typically do not provide or refer to a general formal definition of numerical stability, instead they describe numerical stability informally or intuitively, or define the notion with respect to a specific numerical method. 
% For a formal definition of numerical stability, please refer to \cite{Jong1977TowardsAF}.


% \cite{Bousquet2002StabilityAG} define various notions of stability for learning algorithms with respect to changes in the training dataset. Hypothesis stability is the average variance computed by leave one out error, i.e. how much the function learned by the algorithm will change when a data point in the training set is removed. Pointwise hypothesis stability is very similar to Hypothesis Stability, but it computes the change at only one of the training set point as opposed to the average change. Error Stability measures the change in expected error computed across all sample datasets S. Finally, the strongest notion of stability, Uniform stability, measures the variance in the learning algorithm with respect to the size of the training set. An algorithm is uniformly stable if its stability scales reciprocally to the size of the training set, i.e.: O(1/N), where N is the training set size.
% Similarly to \cite{Franco2017ACS}, we view numerical instability as a sensitivity of output to small variations in inputs or intermediate quantities that drive the output far from the correct value.  

\subsection{Forward and Backward Error}
Numerical stability can be assessed with forward and backward error analysis. Forward Error is the difference between the computed and ground truth result, i.e.: $f(x) - \hat{f}(x)$, which is minimal for numerically stable algorithms. Forward Error is the distance between the true and approximate solution and is often studied in programming languages research fields such as static analysis, formal deduction, or symbolic execution. There are two drivers of forward error: (1) backward error and (2) condition number. Backward error measures the amount of perturbation that causes an approximate solution and is dependent on the implementation of the algorithm. On the other hand, condition number is independent of the algorithm implementation and is instead inherent to the mathematical problem. Therefore, a large forward error that indicates numerical instability can be estimated with the following rule of thumb: Forward Error $\approx$ Backward Error $*$ Condition number \cite{Higham2002AccuracyAS, Fu2015AutomatedBE}. Forward and backward error analysis is useful, because it allows for tracking down the source of numerical error. If the primary driver is backward error, numerical stability can be increased via an improved implementation. However, a large condition number indicates that the problem itself is inherently difficult and rewriting the mathematical formula or using a different algorithm will not be effective.






==> bug.tex <==
\section{Findings: Bugs}
\subsection{Overview and Statistics}
\subsection{Symptoms and Consequences}
Accuracy
Security
Initialization 
It is system and hardware independent
\subsection{Causes}
Where numerical instable code is located?
\begin{itemize}
\item softmax, deep learning library
\end{itemize}

\subsection{Abstraction patterns}


==> detection.tex <==
\section{Detection of Numerical Instabilities with DeepStability}
The idea of the empirical study of numerical vulnerabilities in PyTorch above is to start a database that developers can consult for any known numerical stability problems of the algorithm they wish to implement. To demonstrate the usefulness of this tool, we used DeepStability to identify undetected numerically unstable implementations in Tensorflow.

==> latextemplate.tex <==
 \noindent \fbox{
	\parbox{0.95\linewidth}{\textbf{Answer to RQ2}: The file-level dependency is too coarse for regression testing of the game software. Using the file-level dependency, all states and actions of the MDP are selected. Our fine-grained test dependency, on the other hand, selected much fewer states, actions and traces. 
	}
}

\begin{figure}
%\begin{minipage}{\columnwidth}
	\begin{lstlisting}[commentstyle=\color{blue},
	basicstyle=\footnotesize\ttfamily,
	numbers=right
	]
void dirswitch(char* dir){
  size_t dir_len;	
  (*@\color{red}\underline{- \textbf{if} (dir\_name != NULL) free (dir\_name); }@*) 
  dir_len = strlen (dir);
  if (dir_len > 0 && dir[dir_len-1] == '/') return;
  (*@\color{olive}\underline{+ \textbf{if} (dir\_name != NULL) free (dir\_name);}@*) 
  dir_name=xmalloc(strlen(server_temp_dir)+dir_len+40);
  strcpy(dir_name, dir);
}

int main() {
  while(1){  
    char *cmd;
    //an example failure inducing input: 1st iteration: "Directory", 2nd: "Directory ./", 3rd: "Directory ./"
    read(0, cmd, BUFSIZE);     
    dirswitch(cmd);
  }
}
\end{lstlisting}
\caption{fault signature for cvs-1.11.4 CVE-2003-0015}
\label{cvsex}
%\end{minipage}
\end{figure}

 


\begin{table*}[!t]
    \centering
%\resizebox{\textwidth}{!}{

    \caption{Results of RTS with different test dependencies ($V_1\rightarrow V_2$)}
    % Preview source code for paragraph 0
\resizebox{\textwidth}{!}{
\begin{tabular}{cccccc|ccccc|ccccc}
\hline 
\multirow{2}{*}{Task ID} & \multicolumn{5}{c|}{\#State} & \multicolumn{5}{c|}{\#Action} & \multicolumn{5}{c}{\#Trace}\tabularnewline
\cline{2-16} \cline{3-16} \cline{4-16} \cline{5-16} \cline{6-16} \cline{7-16} \cline{8-16} \cline{9-16} \cline{10-16} \cline{11-16} \cline{12-16} \cline{13-16} \cline{14-16} \cline{15-16} \cline{16-16} 
 & \toolname & AllFile & Art & Meth. & Node & \toolname  & AllFile & Art & Meth. & Node & \toolname  & AllFile & Art & Meth. & Node \tabularnewline
\hline 
\hline 
1 & 0 & 174 & 0 & 0 & 0 & 23 & 689 & 0 & 23 & 0 & 2 & 2 & 0 & 2 & 0\tabularnewline
2 & 0 & 40 & 0 & 0 & 0 & 25 & 71 & 0 & 25 & 0 & 3 & 4 & 0 & 3 & 0\tabularnewline
3 & 0 & 75 & 0 & 0 & 0 & 61 & 143 & 0 & 61 & 0 & 10 & 11 & 0 & 10 & 0\tabularnewline
4 & 6 & 86 & 6 & 0 & 0 & 0 & 186 & 0 & 0 & 0 & 2 & 5 & 2 & 0 & 0\tabularnewline
5 & 0 & 73 & 0 & 0 & 0 & 50 & 224 & 0 & 50 & 0 & 9 & 10 & 0 & 9 & 0\tabularnewline
6 & 0 & 115 & 0 & 0 & 0 & 77 & 228 & 0 & 77 & 0 & 8 & 12 & 0 & 8 & 0\tabularnewline
7 & 0 & 22 & 0 & 0 & 0 & 24 & 34 & 0 & 24 & 0 & 3 & 3 & 0 & 3 & 0\tabularnewline
8 & 0 & 89 & 0 & 0 & 0 & 70 & 197 & 0 & 69 & 2 & 21 & 25 & 0 & 20 & 2\tabularnewline
9 & 3 & 60 & 3 & 0 & 0 & 46 & 119 & 0 & 46 & 0 & 13 & 14 & 2 & 13 & 0\tabularnewline
10 & 0 & 20 & 0 & 0 & 0 & 19 & 34 & 0 & 19 & 0 & 2 & 2 & 0 & 2 & 0\tabularnewline
\hline 
\hline 
Total & 9 & 754 & 9 & 0 & 0 & 395 & 1,925 & 0 & 394 & 2 & 73 & 88 & 4 & 70 & 2\tabularnewline
\hline 
\end{tabular}
}
    \label{tab:rtsv12}
\end{table*}

\begin{table*}[ht]
\centering
\caption{Results of RQ2: Testing code fragments ~\label{tbl:dynTest}}
\resizebox{\textwidth}{!}{
    \begin{tabular}{l||c|c|c|c||c|c|c|c||c|c|c|c||c|c|c|c||c|c|c|c} \hline
    %   \multirow{2}{*}{Projects} & 
    %   \multicolumn{4}{|c||} {Test Cases (exe)} &
    %   \multicolumn{4}{|c||}{Random (valid/pass tests)}  &
    %   \multicolumn{4}{|c||}{Radamsa (valid/pass tests)} &
    %   \multicolumn{4}{|c||}{KLEE (valid/pass tests)} &
    %   \multicolumn{4}{|c}{Summary (valid/pass tests)}
      \multirow{2}{*}{Project} & 
      \multicolumn{4}{|c||}{Executable Tests}  &
      \multicolumn{4}{|c||}{Random (valid/pass)}  &
      \multicolumn{4}{|c||}{Radamsa (valid/pass)} &
      \multicolumn{4}{|c||}{KLEE (valid/pass)} &
      \multicolumn{4}{|c}{Summary of testing (valid/pass)}
      \tabularnewline  \cline{2-21}
                                                                & H    & U   & R  & M  & H      & U      & R    & M    & H      & U     & R   & M   & H      & U     & R    & M    & H        & U      & R    & M \\ \hline\hline
      polymorph-0.4.0                        & 9    & 0   & 0  & 0  & 0/4    & 0      & 0    & 0    & 0/4    & 0     & 0   & 0   & 0/5    & 0     & 0    & 0    & 0/13     & 0      & 0    & 0  \\\hline
      ncompress-4.2.4                        & 14   & 10  & 0  & 0  & 2/4    & 0/2    & 0    & 0    & 1/3    & 0     & 0   & 0   & 2/3    & 0     & 0    & 0    & 5/10     & 0/2    & 0    & 0  \\\hline
      man-1.5h1                              & 33   & 12  & 5  & 1  & 5/18   & 0/7    & 0/4  & 0/1  & 7/9    & 0     & 0/1 & 0   & 5/17   & 0/7   & 0/5  & 0/1  & 17/44    & 0/14   & 0/10 & 0/2  \\\hline
      gzip-1.2.4                             & 24   & 6   & 1  & 2  & 0/16   & 0/4    & 0/1  & 0/2  & 0/13   & 0/1   & 0   & 0   & 0/14   & 0/2   & 0    & 0/2  & 0/43     & 0/7    & 0/1  & 0/4  \\\hline
      bc-1.06                                & 37   & 1   & 0  & 0  & 0/23   & 0/1    & 0    & 0    & 1/22   & 0     & 0   & 0   & 0/22   & 0/1   & 0    & 0    & 1/67     & 0/2    & 0    & 0  \\\hline
      cvs-1.11.4                             & 312  & 61  & 5  & 7  & 9/158  & 3/37   & 0/4  & 0/6  & 10/51  & 3/3   & 0   & 0/1 & 7/126  & 3/15  & 0/3  & 0/5  & 26/335   & 9/55   & 0/7  & 0/12 \\\hline
      squid-2.3.STABLE5                      & 155  & 31  & 0  & 3  & 14/54  & 2/11   & 0    & 0/1  & 20/36  & 2/1   & 0   & 0   & 19/70  & 1/14  & 0    & 0    & 53/160   & 5/26   & 0    & 0/1  \\\hline
      httpd-2.0.48                           & 25   & 18  & 1  & 0  & 0/16   & 0/5    & 0/1  & 0    & 0/3    & 0/2   & 0   & 0   & 0/5    & 0/2   & 0/1  & 0    & 0/24     & 0/9    & 0/2  & 0  \\\hline\hline
      findutils-e6680237                     & 89   & 37  & 4  & 8  & 5/28   & 3/22   & 1/3  & 1/3  & 4/15   & 4/6   & 1/3 & 0/3 & 4/34   & 2/22  & 1/3  & 1/3  & 13/77    & 9/50   & 3/9  & 2/9  \\\hline
      make-0afbbf85                          & 64   & 14  & 0  & 2  & 3/31   & 0/10   & 0    & 0/2  & 2/11   & 0/2   & 0   & 0   & 1/24   & 0/5   & 0    & 0/2  & 6/66     & 0/17   & 0    & 0/4  \\\hline
      grep-c32c0421                          & 109  & 13  & 1  & 0  & 13/66  & 1/9    & 0    & 0    & 17/14  & 1/4   & 0   & 1/0 & 7/63   & 1/5   & 0/1  & 0    & 37/143   & 3/18   & 0/1  & 1/0  \\\hline
      coreutils-0928c241                     & 132  & 68  & 14 & 20 & 5/100  & 1/50   & 0/12 & 0/16 & 7/39   & 1/17  & 0/2 & 0/4 & 5/74   & 1/31  & 0/5  & 0/13 & 17/213   & 3/98   & 0/19 & 0/33 \\\hline\hline
      \multirow{2}{*}{Total}                               & 1003 & 271 & 31 & 43 & 56/518 & 10/158 & 1/25 & 1/31 & 69/220 & 11/36 & 1/6 & 1/8 & 50/457 & 8/104 & 1/18 & 1/26 & 175/1195 & 29/298 & 3/49 & 3/65 \\\cline{2-21}
     & \multicolumn{4}{|c||}{1348} & \multicolumn{4}{|c||}{68/732} & \multicolumn{4}{|c||}{82/270} & \multicolumn{4}{|c||}{60/605} & \multicolumn{4}{|c}{210/1607} \\\hline
    \end{tabular}
}  
\end{table*} 

==> paperstory.tex <==
\section{Paper Outline}

Motivation: why find them in the software repository? 
\begin{itemize}
    \item these unstable methods are not always well documented (why?)
    \item once discovered, it can be reused across ML libraries and across other numerical applications
    \item it has a significant consequence on ML learning algorithms 
    \item in the past, the solutions are typically increasing the precision, but it is not always work?
    \item software repository has software patches that can be used as a reference to fix the code, code patterns can be used to develop tools to detect similar problems, test cases can be reused to test other applications for similar problems
\end{itemize}

contributions:

\begin{itemize}
    \item a catalog of cleaned unstable numerical methods and their solutions
    \item a tool to detect and patch unstable methods in their DL implementations 
    \item patches and bugs found in real-world ML libraries 
    \item open source tool that can report and search unstable numerical methods and their solutions to support reliable programming in ML
\end{itemize}
\subsection{A Motivating Example}

softmax:  unstable version (math), code patterns that can be used to detect other softmax version
(1) why unstable
(2) manifest in code
(3) impact in deep learning end-users 
(4) when it can be triggered: values such as learning rate, weight initialization, data shuffling, the order of training input

solution: mathematically equivalent rewrite: stable version (proof in Appendix)

general applicable: what other places we use softmax in addition to DNN classification?

Goal: 
\begin{itemize}
    \item discover a list of such unstable methods and solutions
    \item detect similar unstable methods in different libraries
\end{itemize}

\subsection{A list of unstable methods and their analysis}

Classifications

\subsection{A tool based on the unstable patterns to discover more of such problems}



==> proof_novel.tex <==
\section{Novel Proof for LogSoftmax}
Logsoftmax is a canonical example of a numerically unstable formula that is commonly used in DL. Prior literature shows how to rewrite the formula to obtain a numerically stable solution, but does not provide proof that the two formulas are mathematically equivalent. To our best knowledge, this is the fist comprehensive proof which shows that step by step. 

LogSoftmax performs softmax followed by the logarithm function and therefore, outputs log probabilities. LogSoftmax is defined as: 
\begin{equation}
    logsoftmax(\vec{x})_i = \frac{log(e^{x_i})}{\sum_{j=1}^{n} e^{x_j}}
\end{equation}

This mathematical formula is numerically unstable and should be implemented as: 
\begin{equation}
    logsoftmax(\vec{x})_i = x_i - max(\vec{x}) -log(\sum_{j=1}^{n} e^{x_j - max(\vec{x})})
\end{equation}

These two equations are mathematically equivalent, which can be proved utilizing the identity: 
\begin{equation}
\label{identity}
    log(\sum_{j=1}^{n} e^{x_j}) = max(\vec{x}) + log(\sum_{j=1}^{n} e^{x_j - max(\vec{x})})
\end{equation}

We first prove the correctness of the identity and then the mathematical equivalence of the numerically stable and unstable logsoftmax formulas.


\begin{proof}
\tiny
    Let $c$ be a scalar constant such that $c = max(x_{1}, ..., x_{n})$
    \begin{flalign*}
        log(\sum_{j=1}^{n} e^{x_j})
        &= max(\vec{x}) + log(\sum_{j=1}^{n} e^{x_j - max(\vec{x})})\\
        &= c + log(\sum_{j=1}^{n} e^{x_j - c}) \\ 
        &= c + log(\sum_{j=1}^{n} e^{x_j} * e^{-c})&&\text{By property $e^{a-b} = e^{a} * e^{b}$}\\
        &= c + log(e^{-c}) + log(\sum_{j=1}^{n} e^{x_j})&&\text{By property $log(ab) = log(a) + log(b)$}\\
        &= c + (-c * log(e)) + log(\sum_{j=1}^{n} e^{x_j})&&\text{By property $log(a^{b} = b * log(a)$}\\
        &= c + (-c(1)) + log(\sum_{j=1}^{n} e^{x_j})&&\text{By property $log(e) = 1$}\\
        &= c - c + log(\sum_{j=1}^{n} e^{x_j})\\
        &= log(\sum_{j=1}^{n} e^{x_j})
    \end{flalign*}
\end{proof} 

\begin{proof}
\tiny
    \begin{flalign*}
        logsoftmax(\vec{x})_i &= \frac{log(e^{x_i})}{\sum_{j=1}^{n} (e^{x_j})}\\
        &= log(e^{x_i}) - log(\sum_{j=1}^{n} e^{x_j})&&\text{By property $log(a/b) = log(a) - log(b)$}\\
        &= x_i * log(e) - log(\sum_{j=1}^{n} e^{x_j})&&\text{By property $log(a^{b}) = b*log(a)$}\\
        &= x_i * (1) - log(\sum_{j=1}^{n} e^{x_j})&&\text{By property $log(e)=1$}\\
        &= x_i - (max(\vec{x}) + log(\sum_{j=1}^{n} e^{x_j - max(\vec{x})}))&&\text{By identity in Equation \ref{identity}}\\
        &= x_i - max(\vec{x}) - log(\sum_{j=1}^{n} e^{x_j - max(\vec{x})})
    \end{flalign*}
\end{proof} 



